Array Languages Make Neural Networks Fast

Modern machine learning frameworks are complex: they are typically organised in multiple layers each of which is written in a different language and they depend on a number of external libraries, but at their core they mainly consist of tensor operations. As array-oriented languages provide perfect abstractions to implement tensor operations, we consider a minimalistic machine learning framework that is shallowly embedded in an array-oriented language and we study its productivity and performance. We do this by implementing a state of the art Convolutional Neural Network (CNN) and compare it against implementations in TensorFlow and PyTorch --- two state of the art industrial-strength frameworks. It turns out that our implementation is 2 and 3 times faster, even after fine-tuning the TensorFlow and PyTorch to our hardware --- a 64-core GPU-accelerated machine. The size of all three CNN specifications is the same, about 150 lines of code. Our mini framework is 150 lines of highly reusable hardware-agnostic code that does not depend on external libraries. The compiler for a host array language automatically generates parallel code for a chosen architecture. The key to such a balance between performance and portability lies in the design of the array language; in particular, the ability to express rank-polymorphic operations concisely, yet being able to do optimisations across them. This design builds on very few assumptions, and it is readily transferable to other contexts offering a clean approach to high-performance machine learning.

==> Makefile <==
SRC := intro.tex \
       background.tex \
       arrays-sac.tex \
       cnn.tex \
       performance.tex \
       related.tex \
       conclusions.tex \
       paper.bib

paper.pdf: paper.tex $(SRC)
	if which latexmk > /dev/null 2>&1 ;\
        then latexmk -pdf -f -pdflatex='pdflatex -halt-on-error' $< ;\
        else pdflatex $< && \
        bibtex $(patsubst %.tex,%,$<) && \
        pdflatex $< ;\
        pdflatex $< ;\
        fi
clean:
	$(RM) *.aux *.log *.out *.vrb paper.pdf \
              *.bbl *.blg *.fdb_latexmk *.toc *.fls *.cut


